Neutrinos Meet Supersymmetry: Quantum Aspects of of Neutrinophysics in Supersymmetric Theories

We address the influence of quantum corrections to neutrino masses and mixings and discuss the possibilities to completely generate the flavor mixing irrespective of any tree-level flavor model. Furthermore, we describe a new class of vacua with a new minimum appearing in the standard Higgs direction. The results hint towards a charge and color breaking global minimum and therefore extend existing bounds at tree-level. Finally, we combine the discussion of vacuum stability in the MSSM with the right-handed neutrino extension. The supersymmetric version of the seesaw mechanism rescues the potential and also does not induce further instabilities neither at the SUSY scale nor at the scale of heavy neutrinos, as long as both scales are well separated. Moreover, we resolve a degeneracy in name space.

==> FrontBackmatter/DirtyTitlepage.tex <==
%*******************************************************
% Little Dirty Titlepage
%*******************************************************
\thispagestyle{empty}
%\pdfbookmark[1]{Titel}{title}
%*******************************************************
\begin{center}
    \spacedlowsmallcaps{\myName} \\ \medskip                        

    \begingroup
        \color{Maroon}\spacedallcaps{\myTitle}
    \endgroup
\end{center}        

